High-Performance Large-Scale Image Recognition Without Normalization

Batch normalization is a key component of most image classification models, but it has many undesirable properties stemming from its dependence on the batch size and interactions between examples. Although recent work has succeeded in training deep ResNets without normalization layers, these models do not match the test accuracies of the best batch-normalized networks, and are often unstable for large learning rates or strong data augmentations. In this work, we develop an adaptive gradient clipping technique which overcomes these instabilities, and design a significantly improved class of Normalizer-Free ResNets. Our smaller models match the test accuracy of an EfficientNet-B7 on ImageNet while being up to 8.7x faster to train, and our largest models attain a new state-of-the-art top-1 accuracy of 86.5%. In addition, Normalizer-Free models attain significantly better performance than their batch-normalized counterparts when finetuning on ImageNet after large-scale pre-training on a dataset of 300 million labeled images, with our best models obtaining an accuracy of 89.2%. Our code is available at https://github.com/deepmind/ deepmind-research/tree/master/nfnets

==> UAGC_algo.tex <==
\begin{algorithm}[H]\small
\caption{Angular SGD.}
  \label{alg:AngSGD}
\begin{algorithmic}
  \STATE {\bfseries Input:} weight matrix $w_t$, learning rate $\eta$,
  weight decay $\lambda$, update core $\rho$, normalizing function $\phi$
  \REPEAT
  \STATE collect gradients $g_t$ via backpropagation
     \STATE $u_t = \rho(g_t)$
     \STATE $w_{t+1} = (\cos(\eta) - \lambda\sin(\eta)) \cdot w_t - \sin(\eta) \cdot\frac{\phi(w_t)}{\phi(w_t)}\cdot u_t$
  \UNTIL{converged}
\end{algorithmic}
\end{algorithm}

==> experiments_to_run.tex <==
1. Try WS at init and BN at init (actnorm) and run ablations at various batch sizes, learning rates, depths.

2. Try just running with skipinit, no WS, if we can get away with the simpler thing, that's good. Compare:

 (a) Skipinit, no WS
 (b) Skipinit + WS
 (c) Variance Downscaling + WS
 (d) Variance downscaling + skipinit + WS
 
 Run the above both w/ our gradient clipping and without
 
 
-For grad clipping: LR sweep at different batch sizes (in neighborhood of predicted LR based on Goyal et al.), we expect to find that at small batch sizes clipping provides no benefit (i.e. you don't need it) but it's necessary at high batches to enable training with the expected learning rate.

-Related to the above: can we train at higher than the goyal LR?


-hidden hyperparameter in BatchNorm is the "ghost batch size", which effectively controls regularization (cite skipinit and ghost BN paper https://arxiv.org/abs/1705.08741)



==> tables/nfresnet_block_ablations.tex <==
\begin{center}
\begin{tabular}{l| l | c | c | c}
\toprule [0.15em]
                           & & BS 256 & BS 1024 & BS 4096 \\
\midrule [0.1em]
\multirow{7}{*}{ResNet50}  & Batch normalization & $76.7 \pm 0.1$ & $76.7 \pm 0.1$ & $76.9 \pm 0.1$ \\
                           & SkipInit & $76.0 \pm 0.1$ & $76.2 \pm 0.2$ & $72.2 \pm 0.3$ \\
                           & + Scaled WS & $76.8 \pm 0.1$ & $77.0 \pm 0.1$ & $76.0 \pm 0.1$ \\
                           & (1) + (2) & $76.9 \pm 0.1 ^\star$ & $77.1 \pm 0.1$ & $75.8 \pm 0.1$ \\
                           & (1) + (2) + (3) & $77.0 \pm 0.1$ & $77.1 \pm 0.0$ & $75.2 \pm 0.1$ \\
                           & (1) + (2) + (4) & $76.9 \pm 0.1$ & $77.0 \pm 0.1$ & $74.8 \pm 0.2 ^\star$ \\
                           & (1)+(2)+(3)+(4) (NF-ResNet) & $76.9 \pm 0.2$ & $77.0 \pm 0.1$ & $76.0 \pm 0.1$ \\
\midrule [0.1em]
\multirow{7}{*}{ResNet200}  & Batch normalization & $79.0 \pm 0.1$ & $79.1 \pm 0.1$ & $79.1 \pm 0.1$  \\
                           & SkipInit & $78.7 \pm 0.1$ & $78.8 \pm 0.1^\star$ & $72.7 \pm 0.2$ \\
                           & + Scaled WS & $79.5 \pm 0.1^\star$ & $79.7 \pm 0.1$ & $78.6 \pm 0.1$ \\
                           & (1) + (2) & --  & -- & -- \\
                           & (1) + (2) + (3) & $79.8 \pm 0.1^\star$ & $79.9 \pm 0.1^\star$ & $77.5 \pm 0.0^\star$ \\
                           & (1) + (2) + (4) & $79.2 \pm 0.1$ & $79.3 \pm 0.1 ^\star$ & $77.1 \pm 0.1$ \\
                           & (1)+(2)+(3)+(4) (NF-ResNet)  & $79.5 \pm 0.2$ & $79.6 \pm 0.1$ & $78.5 \pm 0.1$ \\
\bottomrule[0.15em]
\end{tabular}
\end{center}

